Integer Plane Multiflow Maximisation : Flow-Cut Gap and One-Quarter-Approximation

In this paper, we bound the integrality gap and the approximation ratio for maximum plane multiflow problems and deduce bounds on the flow-cut-gap. Planarity means here that the union of the supply and demand graph is planar. We first prove that there exists a multiflow of value at least half of the capacity of a minimum multicut. We then show how to convert any multiflow into a half-integer one of value at least half of the original multiflow. Finally, we round any half-integer multiflow into an integer multiflow, losing again at most half of the value, in polynomial time, achieving a $1/4$-approximation algorithm for maximum integer multiflows in the plane, and an integer-flow-cut gap of $8$.

==> introduction_ipco_bad.tex <==
\section{Introduction}\label{sec:introduction} 

Given an undirected graph $G=(V,E)$ with edge capacities  $c:E\rightarrow\mathbb{R}_+$, and some pairs of vertices given as edges of the graph $H=(V,F)$, the {\em maximum-multiflow problem} with input $(G,H,c)$, asks for the maximum flow that can be routed in $G$, simultaneously between the endpoints of edges in $F$, respecting the capacities $c$. 

  This is one of many widely studied variants of the multiflow problem. Other popular variants include demand flows, all or nothing flows, unsplittable flows etc. In this paper, we are mainly interested in the integer version of this problem, and the half-integer or fractional versions also occur as tools. When capacities are $1$, the capacity constraint specialises to edge-disjointness, whence the {\em maximum edge disjoint paths problem (MEDP)} between a given set of pairs is a special case; MEDP is NP-Hard to compute for general graphs, even in very restricted settings like when $G$ is a tree \cite{garg1997primal}. 
%and for unbounded $k$ : never used or defined;  and do we say something about bounded k ?  I have paper on that which also works for maximisation, but I think for IPCO we should make our discussion as simple as possible.

The edges in $F$ are called {\em demand edges} (sometimes commodities), those in $E$ are called {\em supply edges}; accordingly, $H=(V,F)$ is  the {\em demand graph}, and $G=(V,E)$ is the {\em supply graph}. If $G+H=(V,E\cup F)$ is planar we call the problem a {\em plane} multiflow problem.  Plane multiflows have been studied for the past forty years, starting with Seymour \cite{seymour1981odd}.  

Let $\mcP_e$ $(e\in F)$ be the set of  paths in $G$ between the endpoints of $e$, and $\mcP:=\cup_{e\in F}\mcP_e$. For $P\in\mcP_e$, the edge $e$ is said to be the {\em demand-edge of $P$}, denoted by $e_P$.   A {\em multiflow}, or for simplicity a {\em flow} in this paper is a function $f:\mcP\rightarrow\mathbb{R}^+$. % the derived function on the edges of $G+H$ (which is in most documents the definition of a flow),  
%$f_{G+H}:E\cup F \rightarrow\mathbb{R}^+$, defined by  $f_{G+H}(e):=\sum_{P\in\mcP:e\in P} f(P)$ if $e\in E$ and $f_{G+H}(e):=\sum_{P\in\mcP_e}f(P)$ if $e\in F$; $f_{G+H}$ is called the {\em total flow} of $f$; it is a linear combination of incident vectors of paths $P\in \mcP$ completed to a circuit, with coefficients $f(P)$. 
The flow $f$ is called {\em feasible}, if $\sum_{\{P\in\mcP:e\in P\}} f(P)\le c(e)$ for all $e\in E$. The {\em value} of a flow $f$ is defined as $|f|:=\sum_{P\in\mcP} f(P)$.

For a path $P\in\mcP$, we refer to $f(P)$ as the {\em flow on $P$}. If the flow on every path is integer or half-integer, we say that the flow is integer or half-integer, respectively. A {\em circuit} is a connected subgraph with all degrees equal to two.

Multiflows (without restrictions on integrality) can be maximised in general, in (strongly) polynomial time \cite[ 70.6, page 1225]{schrijver2003combinatorial} using a linear programming algorithm.

 A {\em multicut} for $(G,H)$ is a set of edges $M\subseteq E$ such that every $P\in\mcP$ contains at least one edge in $M$. \footnote{Given a partition of $V$ so that all edges in $F$ join different classes, the edges of $E$ joining different classes form a multicut. A multicut is inclusion wise minimal if there is at least one edge of $F$ going across each partition.} A multicut is the simplest possible and most natural dual to the maximum multiflow problem. 
 %(also in the precise sense of facets of the ``cone of flows'' generated by $\mcP$).
 
 It is easy to see that the value of any feasible multiflow is smaller than or equal to the capacity of any multicut. Klein, Mathieu and Zhou \cite{klein2015correlation}  prove  that computing the minimum multicut is NP-hard if $G+H$ is planar and also provide a PTAS.
 
 %So a maximum value multiflow -- called simply a {\em maximum multiflow} -- and a  minimum capacity multicut -- called a {\em minimum multicut} --  {\em can both be asymptotically computed in polynomial time}, but without light on their relation so far.
 
 % For a class of instances, the maximum ratio of the minimum multicut over the maximum multiflow is called the $\textbf{flow-cut gap}$ of the class. The {\em integer  flow-cut gap}, or {\em half-integer flow-cut gap} is the ratio of the minimum multicut to the maximum integer,  respectively half-integer,  multiflow.

%{\tt to continue here, with multicuts, ...  def of ratios ... and for this class of instances we prove bounds on the multiflow-multicut gap.}

There is a rich literature on the maximum ratio of a minimum capacity of a multicut over the maximum multiflow. With an abuse of terminology we will call this the  {\em (possibly integer or half-integer) flow-cut gap}, sometimes also restricted to subclasses of problems. This is not to be confused with the same term used for demand problems.  The integer flow-cut gap is $1$ when $G$ is a path and $2$ when $G$ is a tree. For arbitrary $(G,H)$, the flow-cut gap is $\theta(\log |F|)$ \cite{garg1996approximate}. Building on decomposition theorems from Klein, Plotkin and Rao \cite{klein1993excluded}, Tardos and Vazirani~\cite{TV} showed a flow-cut gap of $O(r^3)$ for graphs which do not contain a $K_{r,r}$ minor; note that for $r=3$ this includes the class of planar graphs. A long line of impressive work, culminated in \cite{seguin2011maximum} proving a constant approximation ratio for maximum half-integer flows, which together with ~\cite{TV} implies a constant half-integer flow-cut gap for planar supply graphs. A simple topological obstruction proves that the integer flow-cut gap for planar supply graphs, even when all demand edges  are on one face of the graph,  also called {\em Okamura-Seymour instances},  is $\Omega(|F|)$\cite{garg1997primal}. 

These results are often bounded by the {\em integrality gap} of the multiflow problems for the problem classes, which is the infimum of MAX$/|f|$ over all instances $(G,H,c)$ of the problem class, and where MAX is  the maximum value of an integer multiflow, and  $f$ is a  multiflow for this same input, and
the {\em half-integrality gap} is defined similarly by replacing ``integer'' by ``half-integer'' in the nominator.  A $\rho$-approximation algorithm $(\rho\in\mathbb{R})$ for a maximisation problem is a polynomial algorithm which outputs a solution of value at least $\rho$ times the optimum; $\rho$ is also called the {\em approximation ratio} (or guarantee). 
%It is related to the  integrality gap whenever an integer flow satisfying the gap is found via a polynomial algorithm.

Our first result (Section~\ref{sec:multicuts}, Theorem~\ref{maxflow mincut}) is an upper bound of $2$ for the flow-cut gap (i.e. multicut/multiflow ratio) for plane instances, the missing relation we mentioned.  We prove this by relating multicuts to $2$-edge-connectivity-augmentation  in the plane-dual, and applying a bound of  Williamson, Goemans, Mihail and Vazirani \cite{williamson1995primal} for this problem.

We next show (Section~\ref{sec:half}, Theorem~\ref{thm:half}) how to obtain a half-integer flow from a given (fractional) flow in plane instances, reducing the problem to a linear program with a particular combinatorial structure, and solving it. 

Finally, given any feasible half-integer flow, we show how to extract an integer flow of  value at least half of the original, in polynomial time, using an algorithm that $4$-colors planar graphs efficiently \cite{robertson1996efficiently}. 

These results imply an integrality gap of  $1/2$ for maximum half-integer flows, $1/4$ for maximum integer flows, and the same approximation ratios for each. %a 2-approximation algorithm for minimum multicut for these instances.
In turn, the flow-cut gap of $2$ implies a half-integer flow-cut gap of $4$ and an integer flow-cut gap of $8$ for plane instances. 
% Finally, we provide an example which shows a lower bound of 3/2 on multiflow-multicut gap and 2 on the half-integer multiflow-multicut gap. And integer ? 

A summary of the results completed by lower bounds and open problems are stated in Section~\ref{sec:conclusions}. %TEMPORARY The Appendix  is a guide to some of the tools.
These are the first constant approximation ratios and gaps proved for the studied problems. 
Approximately at the same time as our submission to this
volume, another manuscript was published on Arxiv, proving
constant ratios for the same problems (https://arxiv.org/abs/2001.01715). 


%The above theorems imply a flow-cut gap of 2, a half-integer flow-cut gap of 4 and an integer flow-cut gap of $8$ for plane instances. They also imply a 2-approximation algorithm for maximum half-integer flow, a 4-approximation algorithm for integer flow and a 2-approximation algorithm for minimum multicut for these instances. Finally, we provide an example which shows a lower bound of 3/2 on multiflow-multicut gap and 2 on the half-integer multiflow-multicut gap.

%Note that all these problems as stated above can be solved in polynomial time by using linear programming, but if we add the additional integerity constraints on the flow, all of them become NP-Hard for arbitrary number of demands. If the number of demands is a constant, integer flow problems can be solved in polynomial time by using Graph Minor Theory developed by Robertson and Seymour. The dual to the sum multicommodity flow problem is the cut problem: find a minimum capacity set of edges such that their removal disconnects end points of every demand edge. This is called the multicut problem. The value of maximum total flow is at most the capacity of any multicut. Minimum multicut is NP-Hard even when the supply graph is a tree \cite{garg1997primal}. 








